The Long-Baseline Neutrino Experiment: Exploring Fundamental Symmetries of the Universe

The preponderance of matter over antimatter in the early Universe, the dynamics of the supernova bursts that produced the heavy elements necessary for life and whether protons eventually decay --- these mysteries at the forefront of particle physics and astrophysics are key to understanding the early evolution of our Universe, its current state and its eventual fate. The Long-Baseline Neutrino Experiment (LBNE) represents an extensively developed plan for a world-class experiment dedicated to addressing these questions. LBNE is conceived around three central components: (1) a new, high-intensity neutrino source generated from a megawatt-class proton accelerator at Fermi National Accelerator Laboratory, (2) a near neutrino detector just downstream of the source, and (3) a massive liquid argon time-projection chamber deployed as a far detector deep underground at the Sanford Underground Research Facility. This facility, located at the site of the former Homestake Mine in Lead, South Dakota, is approximately 1,300 km from the neutrino source at Fermilab -- a distance (baseline) that delivers optimal sensitivity to neutrino charge-parity symmetry violation and mass ordering effects. This ambitious yet cost-effective design incorporates scalability and flexibility and can accommodate a variety of upgrades and contributions. With its exceptional combination of experimental configuration, technical capabilities, and potential for transformative discoveries, LBNE promises to be a vital facility for the field of particle physics worldwide, providing physicists from around the globe with opportunities to collaborate in a twenty to thirty year program of exciting science. In this document we provide a comprehensive overview of LBNE's scientific objectives, its place in the landscape of neutrino physics worldwide, the technologies it will incorporate and the capabilities it will possess.

==> insets/matter_effect.tex <==
\begin{insetbox}[frametitle=THE MATTER EFFECT]
\fixme{From a presentation by Smirnov - need to redo for GeV $\nu$}
\includegraphics[width=\textwidth]{figures/matter_effect_smirnov.jpg}
\end{insetbox}


==> insets/neut_osc.tex <==
\begin{insetbox}[frametitle=NEUTRINO OSCILLATIONS]
\fixme{Need to develop a better version of this figure for nue oscillations:}

\includegraphics[width=\textwidth]{figures/nuosc_cartoon.png}

\end{insetbox}


==> insets/proton_decay.tex <==
\begin{insetbox}[frametitle=PROTON DECAY]
\fixme{text taken verbatim from Wikipedia:}

Proton decay, bound neutron decay and similar processes such as
di-nucleon decay and neutron-antineutron oscillation test the apparent
but unexplained conservation law of baryon number. These decays are
already known to be rare based on decades of prior searches, all of
which have produced negative results. If measurable event rates or even 
single-candidate events were to be found, it would be sensible to presume that 
they occurred via unknown virtual processes based on physics beyond
the Standard Model. The impact of demonstrating the existence of a
baryon-number-violating process would be profound.


% Anne changed per Maury 10/29
% In the Standard Model, protons, are theoretically stable because baryon number (quark number) is 
 %conserved. Therefore, protons will not decay into other particles on their own, 
 %because they are the lightest (and therefore least energetic) baryon.
 %Some beyond-the-Standard Model grand unified theories (GUTs)
 %explicitly break the baryon number symmetry, allowing protons to
 %decay via the Higgs particle, magnetic monopoles or new X
 %bosons. Proton decay is one of the few observable effects of the
 %various proposed GUTs. To date, all attempts to observe these events
 %have failed. 
 \includegraphics[width=0.5\textwidth]{figures/proton_decay_knu.png}
\end{insetbox}



==> lbneauthor-payload-authblk.tex <==
% The LBNE author list in authblk format
% This file was generated on March 26, 2014, 8:52 a.m. 
% The collaboration listed is as it was on the date: 2014-03-26.
% Retrieved from: lbne.bnl.gov/web/members/export/?filename=lbneauthor-payload-authblk.tex&amp;date=2014-03-26
% This file was generatd, do not edit this file!
% Contact Maury Goodman for any changes.






\author[85]{C.~Adams}
\author[7]{D.~Adams}
\author[23]{T.~Akiri}
\author[67]{T.~Alion}
\author[25]{K.~Anderson}
\author[40]{C.~Andreopoulos}
\author[25]{M.~Andrews}
\author[33]{I.~Anghel}
\author[14]{J.~C.~C.~d.~Anjos}
\author[36]{M.~Antonello}
\author[46]{E.~Arrieta-Diaz}
\author[74]{M.~Artuso}
\author[74]{J.~Asaadi}
\author[69]{X.~Bai}
\author[56]{B.~Baibussinov}
\author[32]{M.~Baird}
\author[84]{B.~Balantekin}
\author[25]{B.~Baller}
\author[32]{B.~Baptista}
\author[68]{D.~Barker}
\author[81]{G.~Barker}
\author[45]{W.~A.~Barletta}
\author[55]{G.~Barr}
\author[41]{L.~Bartoszek}
\author[76]{A.~Bashyal}
\author[18]{M.~Bass}
\author[13]{V.~Bellini}
\author[58]{P.~A.~Benetti}
\author[18]{B.~E.~Berger}
\author[8]{M.~Bergevin}
\author[25]{E.~Berman}
\author[8]{H.~Berns}
\author[39]{A.~Bernstein}
\author[25]{R.~Bernstein}
\author[30]{B.~Bhandari}
\author[57]{V.~Bhatnagar}
\author[31]{B.~Bhuyan}
\author[49]{J.~Bian}
\author[7]{M.~Bishai}
\author[11]{A.~Blake}
\author[42]{F.~Blaszczyk}
\author[44]{E.~Blaufuss}
\author[71]{B.~Bleakley}
\author[15]{E.~Blucher}
\author[74]{S.~Blusk}
\author[25]{V.~Bocean}
\author[58]{F.~Boffelli}
\author[41]{J.~Boissevain}
\author[35]{T.~Bolton}
\author[48]{M.~Bonesini}
\author[81]{S.~Boyd}
\author[76]{A.~Brandt}
\author[8]{R.~Breedon}
\author[46]{C.~Bromberg}
\author[7]{R.~Brown}
\author[25]{G.~Brunetti}
\author[18]{N.~Buchanan}
\author[75]{B.~Bugg}
\author[2]{J.~Busenitz}
\author[58]{E.~Calligarich}
\author[19]{L.~Camilleri}
\author[9]{G.~Carminati}
\author[19]{R.~Carr}
\author[27]{C.~Castromonte}
\author[85]{F.~Cavanna}
\author[56]{S.~Centro}
\author[25]{A.~Chen}
\author[7]{H.~Chen}
\author[7]{K.~Chen}
\author[18]{D.~Cherdack}
\author[19]{C.~Chi}
\author[25]{S.~Childress}
\author[21]{B.~C.~Choudhary}
\author[40]{G.~Christodoulou}
\author[69]{C.~Christofferson}
\author[85]{E.~Church}
\author[10]{D.~Cline}
\author[72]{T.~Coan}
\author[51]{A.~Cocco}
\author[78]{J.~Coelho}
\author[17]{S.~Coleman}
\author[45]{J.~M.~Conrad}
\author[64]{M.~Convery}
\author[69]{R.~Corey}
\author[69]{L.~Corwin}
\author[4]{J.~Cranshaw}
\author[49]{D.~Cronin-Hennessy}
\author[48]{A.~Curioni}
\author[14]{H.~da~Motta}
\author[65]{T.~Davenne}
\author[33]{G.~S.~Davies}
\author[39]{S.~Dazeley}
\author[76]{K.~De}
\author[53]{A.~de~Gouvea}
\author[55]{J.~K.~de~Jong}
\author[49]{D.~Demuth}
\author[65]{C.~Densham}
\author[7]{M.~Diwan}
\author[4]{Z.~Djurcic}
\author[58]{R.~Dolfini}
\author[7]{J.~Dolph}
\author[4]{G.~Drake}
\author[29]{S.~Dye}
\author[67]{H.~Dyuang}
\author[46]{D.~Edmunds}
\author[41]{S.~Elliott}
\author[2]{M.~Elnimr}
\author[44]{S.~Eno}
\author[82]{S.~Enomoto}
\author[25]{C.~O.~Escobar}
\author[43]{J.~Evans}
\author[58]{A.~Falcone}
\author[73]{L.~Falk}
\author[76]{A.~Farbin}
\author[56]{C.~Farnese}
\author[56]{A.~Fava}
\author[44]{J.~Felde}
\author[2]{S.~Fernandes}
\author[58]{F.~Ferroni}
\author[84]{F.~Feyzi}
\author[53]{L.~Fields}
\author[37]{A.~Finch}
\author[65]{M.~Fitton}
\author[85]{B.~Fleming}
\author[23]{J.~Fowler}
\author[32]{W.~Fox}
\author[41]{A.~Friedland}
\author[25]{S.~Fuess}
\author[38]{B.~Fujikawa}
\author[78]{H.~Gallagher}
\author[28]{R.~Gandhi}
\author[41]{G.~Garvey}
\author[38]{V.~M.~Gehman}
\author[7]{G.~d.~Geronimo}
\author[56]{D.~Gibin}
\author[7]{R.~Gill}
\author[27]{R.~A.~Gomes}
\author[4]{M.~C.~Goodman}
\author[68]{J.~Goon}
\author[60]{N.~Graf}
\author[64]{M.~Graham}
\author[50]{R.~Gran}
\author[8]{C.~Grant}
\author[37]{N.~Grant}
\author[25]{H.~Greenlee}
\author[84]{L.~Greenler}
\author[59]{S.~Grullon}
\author[41]{E.~Guardincerri}
\author[4]{V.~Guarino}
\author[80]{E.~Guarnaccia}
\author[24]{G.~Guedes}
\author[85]{R.~Guenette}
\author[56]{A.~Guglielmi}
\author[12]{M.~M.~Guzzo}
\author[50]{A.~T.~Habig}
\author[7]{R.~W.~Hackenburg}
\author[76]{H.~Hadavand}
\author[25]{A.~Hahn}
\author[81]{M.~Haigh}
\author[41]{T.~Haines}
\author[75]{T.~Handler}
\author[7]{S.~Hans}
\author[73]{J.~Hartnell}
\author[18]{J.~Harton}
\author[25]{R.~Hatcher}
\author[75]{A.~Hatzikoutelis}
\author[25]{S.~Hays}
\author[6]{E.~Hazen}
\author[70]{M.~Headley}
\author[25]{A.~Heavey}
\author[85]{K.~Heeger}
\author[70]{J.~Heise}
\author[44]{R.~Hellauer}
\author[43]{J.~Hewes}
\author[23]{A.~Himmel}
\author[18]{M.~Hogan}
\author[12]{P.~Holanda}
\author[79]{A.~Holin}
\author[35]{G.~Horton-Smith}
\author[25]{J.~Howell}
\author[25]{P.~Hurh}
\author[46]{J.~Huston}
\author[25]{J.~Hylen}
\author[42]{R.~Imlay}
\author[42]{J.~Insler}
\author[58]{G.~Introzzi}
\author[7]{Z.~Isvan}
\author[76]{C.~Jackson}
\author[44]{J.~Jacobsen}
\author[7]{D.~E.~Jaffe}
\author[25]{C.~James}
\author[80]{C.~Jen}
\author[25]{M.~Johnson}
\author[16]{R.~Johnson}
\author[17]{R.~Johnson}
\author[17]{S.~Johnson}
\author[18]{W.~Johnston}
\author[25]{J.~Johnstone}
\author[45]{B.~J.~Jones}
\author[25]{H.~Jostlein}
\author[25]{T.~Junk}
\author[38]{R.~Kadel}
\author[50]{K.~Kaess}
\author[19]{G.~Karagiorgi}
\author[82]{J.~Kaspar}
\author[45]{T.~Katori}
\author[25]{B.~Kayser}
\author[6]{E.~Kearns}
\author[59]{P.~Keener}
\author[12]{E.~Kemp}
\author[7]{S.~H.~Kettell}
\author[25]{M.~Kirby}
\author[59]{J.~Klein}
\author[25]{G.~Koizumi}
\author[77]{S.~Kopp}
\author[37]{L.~Kormos}
\author[9]{W.~Kropp}
\author[66]{V.~A.~Kudryavtsev}
\author[57]{A.~Kumar}
\author[29]{J.~Kumar}
\author[42]{T.~Kutter}
\author[13]{F.~La~Zia}
\author[59]{K.~Lande}
\author[22]{C.~Lane}
\author[77]{K.~Lang}
\author[7]{F.~Lanni}
\author[45]{R.~Lanza}
\author[59]{T.~Latorre}
\author[29]{J.~Learned}
\author[41]{D.~Lee}
\author[10]{K.~Lee}
\author[25]{Q.~Li}
\author[7]{S.~Li}
\author[7]{Y.~Li}
\author[23]{Z.~Li}
\author[67]{J.~Libo}
\author[6]{S.~Linden}
\author[7]{J.~Ling}
\author[80]{J.~Link}
\author[7]{L.~Littenberg}
\author[30]{H.~Liu}
\author[41]{Q.~Liu}
\author[72]{T.~Liu}
\author[54]{J.~Losecco}
\author[41]{W.~Louis}
\author[25]{B.~Lundberg}
\author[25]{T.~Lundin}
\author[76]{J.~Lundy}
\author[26]{A.~A.~Machado}
\author[8]{C.~Maesano}
\author[4]{S.~Magill}
\author[7]{G.~Mahler}
\author[4]{D.~Malon}
\author[52]{S.~Malys}
\author[13]{F.~Mammoliti}
\author[21]{S.~K.~Mandal}
\author[78]{A.~Mann}
\author[25]{P.~Mantsch}
\author[25]{A.~Marchionni}
\author[7]{W.~Marciano}
\author[80]{C.~Mariani}
\author[29]{J.~Maricic}
\author[17]{A.~Marino}
\author[49]{M.~Marshak}
\author[11]{J.~Marshall}
\author[29]{S.~Matsuno}
\author[41]{C.~Mauger}
\author[40]{K.~Mavrokoridis}
\author[78]{N.~Mayer}
\author[40]{N.~McCauley}
\author[25]{E.~McCluskey}
\author[61]{K.~McDonald}
\author[63]{K.~McFarland}
\author[35]{D.~McKee}
\author[83]{R.~McKeown}
\author[71]{R.~McTaggart}
\author[77]{R.~Mehdiyev}
\author[68]{D.~Mei}
\author[58]{A.~Menegolli}
\author[56]{G.~Meng}
\author[10]{Y.~Meng}
\author[2]{D.~Mertins}
\author[32]{M.~Messier}
\author[42]{W.~Metcalf}
\author[29]{R.~Milincic}
\author[49]{W.~Miller}
\author[41]{G.~Mills}
\author[67]{S.~R.~Mishra}
\author[25]{N.~Mokhov}
\author[58]{C.~Montanari}
\author[25]{D.~Montanari}
\author[25]{C.~Moore}
\author[25]{J.~Morfin}
\author[81]{B.~Morgan}
\author[7]{W.~Morse}
\author[45]{Z.~Moss}
\author[1]{C.~A.~Moura}
\author[32]{S.~Mufson}
\author[64]{D.~Muller}
\author[32]{J.~Musser}
\author[60]{D.~Naples}
\author[62]{J.~Napolitano}
\author[59]{M.~Newcomer}
\author[79]{R.~Nichol}
\author[65]{T.~Nicholls}
\author[32]{E.~Niner}
\author[25]{B.~Norris}
\author[37]{J.~Nowak}
\author[37]{H.~O'Keeffe}
\author[12]{R.~Oliveira}
\author[78]{T.~Olson}
\author[46]{B.~Page}
\author[29]{S.~Pakvasa}
\author[85]{O.~Palamara}
\author[4]{J.~Paley}
\author[60]{V.~Paolone}
\author[25]{V.~Papadimitriou}
\author[76]{S.~Park}
\author[7]{Z.~Parsa}
\author[85]{K.~Partyka}
\author[84]{B.~Paulos}
\author[41]{Z.~Pavlovic}
\author[73]{S.~Peeters}
\author[79]{A.~Perch}
\author[63]{G.~Perdue}
\author[66]{J.~D.~Perkin}
\author[67]{R.~Petti}
\author[69]{A.~Petukhov}
\author[56]{F.~Pietropaolo}
\author[25]{R.~Plunkett}
\author[25]{C.~Polly}
\author[25]{S.~Pordes}
\author[7]{M.~Potekhin}
\author[13]{R.~Potenza}
\author[45]{A.~Prakash}
\author[25]{O.~Prokofiev}
\author[7]{X.~Qian}
\author[25]{J.~L.~Raaf}
\author[7]{V.~Radeka}
\author[25]{I.~Rakhno}
\author[81]{Y.~Ramachers}
\author[25]{R.~Rameika}
\author[41]{J.~Ramsey}
\author[58]{A.~Rappoldi}
\author[58]{G.~Raselli}
\author[37]{P.~Ratoff}
\author[76]{S.~Ravindra}
\author[25]{B.~Rebel}
\author[2]{J.~Reichenbacher}
\author[25]{D.~Reitzner}
\author[7]{S.~Rescia}
\author[66]{M.~Richardson}
\author[41]{K.~Rielage}
\author[25]{K.~Riesselmann}
\author[66]{M.~Robinson}
\author[64]{L.~Rochester}
\author[41]{M.~Ronquest}
\author[29]{M.~Rosen}
\author[58]{M.~Rossella}
\author[26]{C.~Rubbia}
\author[25]{R.~Rucinski}
\author[57]{S.~Sahijpal}
\author[4]{H.~Sahoo}
\author[47]{P.~Sala}
\author[58]{D.~Salmiera}
\author[7]{N.~Samios}
\author[33]{M.~Sanchez}
\author[47]{A.~Scaramelli}
\author[53]{H.~Schellman}
\author[25]{R.~Schmitt}
\author[15]{D.~Schmitz}
\author[78]{J.~Schneps}
\author[23]{K.~Scholberg}
\author[36]{E.~Segreto}
\author[59]{S.~Seibert}
\author[25]{L.~Sexton-Kennedy}
\author[19]{M.~Shaevitz}
\author[25]{P.~Shanahan}
\author[7]{R.~Sharma}
\author[25]{T.~Shaw}
\author[7]{N.~Simos}
\author[5]{V.~Singh}
\author[41]{G.~Sinnis}
\author[19]{W.~Sippach}
\author[74]{T.~Skwarnicki}
\author[9]{M.~Smy}
\author[9]{H.~Sobel}
\author[74]{M.~Soderberg}
\author[7]{J.~Sondericker}
\author[41]{W.~Sondheim}
\author[16]{A.~Sousa}
\author[66]{N.~J.~Spooner}
\author[25]{M.~Stancari}
\author[2]{I.~Stancu}
\author[36]{D.~Stefan}
\author[25]{A.~Stefanik}
\author[7]{J.~Stewart}
\author[74]{S.~Stone}
\author[25]{J.~Strait}
\author[15]{M.~Strait}
\author[25]{S.~Striganov}
\author[44]{G.~Sullivan}
\author[29]{Y.~Sun}
\author[4]{L.~Suter}
\author[67]{A.~Svenson}
\author[8]{R.~Svoboda}
\author[20]{B.~Szczerbinska}
\author[85]{A.~Szelc}
\author[8]{M.~Szydagis}
\author[43]{S.~S\"oldner-Rembold}
\author[4]{R.~Talaga}
\author[73]{M.~Tamsett}
\author[25]{S.~Tariq}
\author[32]{R.~Tayloe}
\author[41]{C.~Taylor}
\author[70]{D.~Taylor}
\author[10]{A.~Teymourian}
\author[7]{H.~Themann}
\author[66]{M.~Thiesse}
\author[79]{J.~Thomas}
\author[66]{L.~F.~Thompson}
\author[11]{M.~Thomson}
\author[7]{C.~Thorn}
\author[65]{M.~Thorpe}
\author[67]{X.~Tian}
\author[69]{D.~Tiedt}
\author[18]{W.~Toki}
\author[82]{N.~Tolich}
\author[58]{M.~Torti}
\author[45]{M.~Toups}
\author[40]{C.~Touramanis}
\author[8]{M.~Tripathi}
\author[25]{I.~Tropin}
\author[64]{Y.~Tsai}
\author[38]{C.~Tull}
\author[42]{M.~Tzanov}
\author[32]{J.~Urheim}
\author[52]{S.~Usman}
\author[34]{M.~Vagins}
\author[3]{G.~A.~Valdiviesso}
\author[59]{R.~Van~Berg}
\author[41]{R.~Van~de~Water}
\author[4]{P.~Van~Gemmeren}
\author[56]{F.~Varanini}
\author[29]{G.~Varner}
\author[25]{K.~Vaziri}
\author[25]{G.~Velev}
\author[56]{S.~Ventura}
\author[36]{C.~Vignoli}
\author[7]{B.~Viren}
\author[84]{D.~Wahl}
\author[73]{A.~Waldron}
\author[23]{C.~W.~Walter}
\author[10]{H.~Wang}
\author[83]{W.~Wang}
\author[66]{T.K.~Warburton}
\author[18]{D.~Warner}
\author[18]{R.~Wasserman}
\author[76]{B.~Watson}
\author[55]{A.~Weber}
\author[68]{W.~Wei}
\author[69]{D.~Wells}
\author[15]{M.~Wetstein}
\author[76]{A.~White}
\author[41]{H.~White}
\author[30]{L.~Whitehead}
\author[32]{D.~Whittington}
\author[70]{J.~Willhite}
\author[18]{R.~J.~Wilson}
\author[10]{L.~Winslow}
\author[67]{K.~Wood}
\author[7]{E.~Worcester}
\author[7]{M.~Worcester}
\author[33]{T.~Xin}
\author[41]{K.~Yarritu}
\author[72]{J.~Ye}
\author[7]{M.~Yeh}
\author[7]{B.~Yu}
\author[76]{J.~Yu}
\author[17]{T.~Yuan}
\author[58]{A.~Zani}
\author[25]{G.~P.~Zeller}
\author[7]{C.~Zhang}
\author[68]{C.~Zhang}
\author[17]{E.~D.~Zimmerman}
\author[25]{R.~Zwaska}



\affil[1]{\mbox{ABC Federal University, Santo Andr\'e \textendash SP, 09210-580, Brazil}}

\affil[2]{\mbox{Univ. of Alabama (Tuscaloosa), Tuscaloosa, AL 35487-0324, USA}}

\affil[3]{\mbox{Univ. Federal de Alfenas em Po\c cos de Caldas, 11999, CEP 37715-900 Po\c cos de Caldas-MG, Brazil}}

\affil[4]{\mbox{Argonne National Lab., Argonne, IL 60439, USA}}

\affil[5]{\mbox{Banaras Hindu University, Dept. of Physics, Varanasi UP 221005, India}}

\affil[6]{\mbox{Boston University, Boston, MA 02215, USA}}

\affil[7]{\mbox{Brookhaven National Lab., Upton, NY 11973-5000, USA}}

\affil[8]{\mbox{Univ. of California (Davis), Davis, CA 95616, USA}}

\affil[9]{\mbox{Univ. of California (Irvine), Irvine, CA 92697-4575, USA}}

\affil[10]{\mbox{Univ. of California (Los Angeles), Los Angeles, CA 90095-1547, USA}}

\affil[11]{\mbox{Univ. of Cambridge, JJ Thomson Avenue, Cambridge CB3 0HE, UK}}

\affil[12]{\mbox{Univ. de Campinas, Av. S\'ergio Buarque de Holanda, 777 CEP 13083-859 Campinas-SP, Brazil}}

\affil[13]{\mbox{Univ. di Catania, Corso Italia, I-95129 Catania, Italy}}

\affil[14]{\mbox{Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, BR-22290-180, Brazil}}

\affil[15]{\mbox{Univ. of Chicago, Chicago, IL 60637-1434, USA}}

\affil[16]{\mbox{Univ. of Cincinnati, Cincinnati, OH 45221-0011, USA}}

\affil[17]{\mbox{Univ. of Colorado, Boulder, CO 80309, USA}}

\affil[18]{\mbox{Colorado State University, Fort Collins, CO 80523, USA}}

\affil[19]{\mbox{Columbia University, New York, NY 10027, USA}}

\affil[20]{\mbox{Dakota State University, Madison, SD 57042, USA}}

\affil[21]{\mbox{Univ. of Delhi, Department of Physics and Astrophysics, Delhi 110007, India}}

\affil[22]{\mbox{Drexel University, Philadelphia, PA 19104, USA}}

\affil[23]{\mbox{Duke University, Durham, NC 27706, USA}}

\affil[24]{\mbox{Univ. Estadual de Feira de Santana, 44036-900, Feira de Santana-BA, Brazil}}

\affil[25]{\mbox{Fermi National Accelerator Lab, Batavia, IL 60510-0500, USA}}

\affil[26]{\mbox{INFN, Laboratori Nazionali del Gran Sasso, I-67010 Assergi, AQ, Italy}}

\affil[27]{\mbox{Univ. Federal de Goias, Goiania, Goias, Brazil}}

\affil[28]{\mbox{Harish-Chandra Research Institute, Jhunsi, Allahabad 211 019, India}}

\affil[29]{\mbox{Univ. of Hawaii, Honolulu, HI 96822-2219, USA}}

\affil[30]{\mbox{Univ. of Houston, Houston, TX 77204, USA}}

\affil[31]{\mbox{Indian Institute of Technology Guwahati, Guwahati, 781 039, India}}

\affil[32]{\mbox{Indiana University, Bloomington, IN 47405-7105, USA}}

\affil[33]{\mbox{Iowa State University, Ames, IO 50011, USA}}

\affil[34]{\mbox{Kavli IPMU, Univ. of Tokyo, Kashiwa Shi, Chiba 277-8568, Japan}}

\affil[35]{\mbox{Kansas State University, Manhattan, KS 66506, USA}}

\affil[36]{\mbox{Laboratori Nazionali del Gran Sasso, I-67010 Assergi, AQ, Italy}}

\affil[37]{\mbox{Lancaster University, Bailrigg, Lancaster LA1 4YB, UK}}

\affil[38]{\mbox{Lawrence Berkeley National Lab., Berkeley, CA 94720-8153, USA}}

\affil[39]{\mbox{Lawrence Livermore National Lab., Livermore, CA 94551, USA}}

\affil[40]{\mbox{Univ. of Liverpool, L69 7ZE, Liverpool, UK}}

\affil[41]{\mbox{Los Alamos National Laboratory, Los Alamos, NM 87545, USA}}

\affil[42]{\mbox{Louisiana State University, Baton Rouge, LA 70803-4001, USA}}

\affil[43]{\mbox{Univ. of Manchester, Oxford Road, Manchester M13 9PL, UK}}

\affil[44]{\mbox{Univ. of Maryland, College Park, MD 20742-4111, USA}}

\affil[45]{\mbox{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}}

\affil[46]{\mbox{Michigan State University, East Lansing, MI 48824, USA}}

\affil[47]{\mbox{Univ. di Milano, INFN Sezione di Milano, I-20133 Milano, Italy}}

\affil[48]{\mbox{Univ. of Milano and INFN Sezione di Milano Bicocca, Piazza della Scienza 3, 20126 Milano, Italy}}

\affil[49]{\mbox{Univ. of Minnesota, Minneapolis, MN 55455, USA}}

\affil[50]{\mbox{Univ. of Minnesota (Duluth), Duluth, MN 55812, USA}}

\affil[51]{\mbox{Univ. di Napoli, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy}}

\affil[52]{\mbox{National Geospatial-Intelligence Agency, Reston, VA 20191, USA}}

\affil[53]{\mbox{Northwestern University, Evanston, Il 60208, USA}}

\affil[54]{\mbox{Univ. of Notre Dame, Notre Dame, IN 46556-5670, USA}}

\affil[55]{\mbox{Univ. of Oxford, Oxford, OX1 3RH, UK}}

\affil[56]{\mbox{Univ. of Padova, Dip. Fisica e Astronomia G. Galilei and INFN Sezione di
Padova, I-35131 Padova, Italy}}

\affil[57]{\mbox{Panjab University, Chandigarh, 160014 U.T., India}}

\affil[58]{\mbox{Univ. of Pavia, INFN Sezione di Pavia, I-27100 Pavia, Italy}}

\affil[59]{\mbox{Univ. of Pennsylvania, Philadelphia, PA 19104-6396, USA}}

\affil[60]{\mbox{Univ. of Pittsburgh, Pittsburgh, PA 15260, USA}}

\affil[61]{\mbox{Princeton University, Princeton, New Jersey 08544-0708, USA}}

\affil[62]{\mbox{Rensselaer Polytechnic Inst., Troy, NY 12180-3590, USA}}

\affil[63]{\mbox{Univ. of Rochester, Rochester, NY 14627-0171, USA}}

\affil[64]{\mbox{SLAC National Acceleratory Laboratory, Menlo Park, CA 94025, USA}}

\affil[65]{\mbox{STFC Rutherford Appleton Laboratory, Harwell Oxford, Didcot OX11 0QX, UK}}

\affil[66]{\mbox{Univ. of Sheffield, Sheffield, S3 7RH, UK}}

\affil[67]{\mbox{Univ. of South Carolina, Columbia, SC 29208, USA}}

\affil[68]{\mbox{Univ. of South Dakota, Vermillion, SD 57069, USA}}

\affil[69]{\mbox{South Dakota School of Mines and Technology, Lead, SD 57754, USA}}

\affil[70]{\mbox{South Dakota Science And Technology Authority, Lead, SD 57754, USA}}

\affil[71]{\mbox{South Dakota State University, Brookings, SD 57007, USA}}

\affil[72]{\mbox{Southern Methodist University, Dallas, TX 75275, USA}}

\affil[73]{\mbox{Univ. of Sussex, Brighton, BN1 9RH, UK}}

\affil[74]{\mbox{Syracuse University, Syracuse, NY 13244-1130, USA}}

\affil[75]{\mbox{Univ. of Tennessee, Knoxville, TN, USA}}

\affil[76]{\mbox{Univ. of Texas (Arlington), Arlington, TX 76019, USA}}

\affil[77]{\mbox{Univ. of Texas (Austin), Austin, TX 78712-0264, USA}}

\affil[78]{\mbox{Tufts University, Medford, MA 02155, USA}}

\affil[79]{\mbox{University College London, London, WC1E 6BT, UK}}

\affil[80]{\mbox{Virginia Tech., Blacksburg, VA 24061-0435, USA}}

\affil[81]{\mbox{Univ. of Warwick, Coventry CV4 7AL, UK}}

\affil[82]{\mbox{Univ. of Washington, Seattle, WA 98195-1560, USA}}

\affil[83]{\mbox{College of William and Mary, Williamsburg, VA 23187-8795, USA}}

\affil[84]{\mbox{Univ. of Wisconsin, Madison, WI 53706, USA}}

\affil[85]{\mbox{Yale University, New Haven, CT 06520, USA}}





==> lbnepaper/draft.tex <==
% Include this to produce a draft version on the document.
\usepackage[pagewise]{lineno}
\linenumbers
\renewcommand{\fixme}[1]{\textbf{FIXME:} \textit{#1}}
\renewcommand{\lbnepagestyle}{glossy}

% show \label and other keys in the margin to make it easier for
% editors to add \ref and other references.
\usepackage[color]{showkeys}
% Add a DRAFT watermark
\usepackage{draftwatermark}
\SetWatermarkText{DRAFT}
\SetWatermarkScale{1}
\SetWatermarkLightness{0.95}


==> lbnepaper/insetbox.tex <==
% \include{lbnepaper/insetbox.tex}
%
% provides an "inset" or "sidebar" box.
% \begin{insetbox}[frametitle=The frame title}
%   ...content...
% \end{insetbox}

\usepackage[xcolor,framemethod=tikz,nobreak=true]{mdframed}
\usetikzlibrary{shadows}

% An "inset" frame for highlighting some specific point.  Use the
% "insetbox" frame with a "[frametitle=The Inset Title]" option to
% provide a title.
\mdfdefinestyle{insetstyle}{frametitle=MISSING TITLE}
\mdfapptodefinestyle{insetstyle}{linecolor=blue}
\mdfapptodefinestyle{insetstyle}{roundcorner=10pt}
\mdfapptodefinestyle{insetstyle}{innerlinewidth=1pt}
\mdfapptodefinestyle{insetstyle}{innerlinecolor=black}
\mdfapptodefinestyle{insetstyle}{middlelinewidth=2pt}
\mdfapptodefinestyle{insetstyle}{middlelinecolor=blue}
\mdfapptodefinestyle{insetstyle}{outerlinewidth=2pt}
\mdfapptodefinestyle{insetstyle}{outerlinecolor=blue!1}
\mdfapptodefinestyle{insetstyle}{backgroundcolor=blue!8}
\mdfapptodefinestyle{insetstyle}{apptotikzsetting={%
\tikzset{mdfbackground/.append style ={%
top color=orange!30!white,
bottom color=orange!80!black}}}}
% this one above does the gradient in title and main backgrounds
\mdfapptodefinestyle{insetstyle}{innerleftmargin=10pt}
\mdfapptodefinestyle{insetstyle}{innerrightmargin=10pt}
\mdfapptodefinestyle{insetstyle}{innertopmargin=20pt}
\mdfapptodefinestyle{insetstyle}{innerbottommargin=10pt}
\mdfapptodefinestyle{insetstyle}{shadow=true}
\mdfapptodefinestyle{insetstyle}{shadowsize=10pt}
\mdfapptodefinestyle{insetstyle}{shadowcolor=gray!40}

\mdfapptodefinestyle{insetstyle}{frametitlefont=\normalfont\ttfamily}
\mdfapptodefinestyle{insetstyle}{frametitlealignment=\centering}
\mdfapptodefinestyle{insetstyle}{frametitlerule=true}
\newmdenv[style=insetstyle]{insetbox}

